Checking Computations of Formal Method Tools - A Secondary Toolchain for ProB

We present the implementation of pyB, a predicate - and expression - checker for the B language. The tool is to be used for a secondary tool chain for data validation and data generation, with ProB being used in the primary tool chain. Indeed, pyB is an independent cleanroom-implementation which is used to double-check solutions generated by ProB, an animator and model-checker for B specifications. One of the major goals is to use ProB together with pyB to generate reliable outputs for high-integrity safety critical applications. Although pyB is still work in progress, the ProB/pyB toolchain has already been successfully tested on various industrial B machines and data validation tasks.

==> eptcsdata.tex <==
\providecommand{\firstpage}{93}
\providecommand{\publicationstatus}{Dubois C., Giannakopoulou D., Méry D. (Eds): Formal Integrated\\Development Environment 2014 (F-IDE 2014)\\
EPTCS 149, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.149.9}{10.4204/EPTCS.149.9}}
\pdfoutput=1

